RECALL: Rehearsal-free Continual Learning for Object Classification

Convolutional neural networks show remarkable results in classification but struggle with learning new things on the fly. We present a novel rehearsal-free approach, where a deep neural network is continually learning new unseen object categories without saving any data of prior sequences. Our approach is called RECALL, as the network recalls categories by calculating logits for old categories before training new ones. These are then used during training to avoid changing the old categories. For each new sequence, a new head is added to accommodate the new categories. To mitigate forgetting, we present a regularization strategy where we replace the classification with a regression. Moreover, for the known categories, we propose a Mahalanobis loss that includes the variances to account for the changing densities between known and unknown categories. Finally, we present a novel dataset for continual learning, especially suited for object recognition on a mobile robot (HOWS-CL-25), including 150,795 synthetic images of 25 household object categories. Our approach RECALL outperforms the current state of the art on CORe50 and iCIFAR-100 and reaches the best performance on HOWS-CL-25.

==> chapters/ablationStudies.tex <==
As \OURAPPROACH is so fast to train, it was possible to do several ablation studies.
In the following, we present hyperparameters, which have a strong influence on the results. 

\input{tables/ablation_studies}

\paragraph{Activation function}

In our approach, different activation functions are tested, see \cref{tab_ablation_studies}.
SIREN proposed by Sitzmann \etal \cite{Sitzmann2020} performs best for both datasets.
In the case of \DLRDataset ReLU performs nearly as well.
%Furthermore, the activation functions Identity, ReLU and SIREN performed better on both datasets than the other evaluated activation functions.
%As the linear function also worked, it can be assumed, that the feature values, resulting from the feature extraction network are linearly separable. %, which might be the case, as the backbone already uses ReLU to solve non-linear approximations.
%Furthermore, the results in our experiments, when using the identity function, are improved by applying a batch normalization. 
%In our experiments the ReLU activation function leads to one of the best results, except if it is combined with batch normalization.	
Even though the SIREN activation function has been successfully used in reconstruction tasks, it works best in our tests.
But, as highlighted in their paper, it highly depends on the initialization values, which is controlled by the first and hidden omega values.

\TODO{check omega names in paper}
\TODO{Gefällt mir so noch nicht..}

\paragraph{Feature extraction network}

We further evaluated the influence of the backbone on the performance, see \cref{tab_ablation_studies}.
As \DLRDataset is a category classification dataset, we assume that more advanced CNNs have an improved accuracy in contrast to \coreFifty, which is an instance-classification dataset.
It can also be seen that ResNet50 proposed by He \etal \cite{He2016} works better than the second version ResNet50V2 also proposed by He \etal \cite{He2016a}.
On the \coreFifty dataset ResNet50 outperforms every other tested backbone.
These results have been partly confirmed by other papers like Maltoni \etal \cite{Maltoni2019}, where they also found that ResNet50 outperformed GoogLeNet, proposed by Szegedy \etal \cite{Szegedy2015} on the \coreFifty dataset.

\paragraph{Using different heads per sequence}

\Cref{tab_ablation_studies} shows that using a different head per sequence improves the results.
Especially for the \coreFifty dataset, as the separation of different sequences reduces the possible influence the training of new output values have on the first layer.

